Counting HyperGraphlets via Color Coding: a Quadratic Barrier and How to Break It

We study the problem of counting $k$-hypergraphlets, an interesting but surprisingly ignored primitive, with the aim of understanding whether efficient algorithms exist. To this end, we consider color coding, a well-known technique for approximately counting $k$-graphlets in graphs. Our first result is that, on hypergraphs, color coding encounters a quadratic barrier: under the Orthogonal Vector Conjecture, no implementation can run in sub-quadratic time in the input size. We then introduce a simple property, $(\alpha,\beta)$-niceness, that hypergraphs from real-world datasets appear to satisfy for small values of $\alpha$ and $\beta$. Intuitively, an $(\alpha,\beta)$-nice hypergraph can be split into two sub-hypergraphs having respectively rank at most $\alpha$ and degree at most $\beta$. By applying different techniques to each sub-hypergraph and carefully combining the outputs, we show how to run color coding in time $2^{O(k)} \cdot (2^\beta |V| + \alpha^k |E| + \alpha^2 \beta \|H\|)$, where $H=(V,E)$ is the input hypergraph. Afterwards, we can sample colorful $k$-hypergraphlets uniformly in expected $k^{O(k)} \cdot (\beta^2 + \ln |V|)$ time per sample. Experiments on real-world hypergraphs show that our algorithm significantly outperforms the naive quadratic algorithm, sometimes by more than an order of magnitude.

==> figures/frequencies/K4_table_resized.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccc}
\hline
& AR & AX & GP & SE & MA & RH & SA \\
\hline
A & 0.0175 & 0.3605 & 0.1136 & 0.3281 & 0.3258 & 0.0692 & 0.2936 \\
% ...
T & 0.0000 & 0.0008 & 0.0016 & 0.0012 & 0.0000 & 0.0266 & 0.0000 \\
\hline
\end{tabular}
}

==> figures/frequencies/k3_table.tex <==
\begin{tabular}{lccccccc}
\hline
Motif & AR & AX & GP & SE & MA & RH & SA \\
\hline
A & 0.9501 & 0.5197 & 0.7494 & 0.5463 & 0.6385 & 0.2323 & 0.2526 \\
B & 0.0156 & 0.2841 & 0.0782 & 0.2784 & 0.3472 & 0.1682 & 0.7437 \\
C & 0.0075 & 0.1665 & 0.0889 & 0.1372 & 0.0116 & 0.3566 & 0.0037 \\
D & 0.0029 & 0.0183 & 0.0405 & 0.0172 & 0.0004 & 0.1734 & 0.0000 \\
E & 0.0228 & 0.0113 & 0.0346 & 0.0203 & 0.0021 & 0.0481 & 0.0001 \\
F & 0.0012 & 0.0002 & 0.0083 & 0.0007 & 0.0000 & 0.0215 & 0.0000 \\
\hline
\end{tabular}

==> pgf-hypergraph.tex <==
\def\hgrotate#1{
  % Rotate input point by 90 degrees counter-clockwise.
  \newdimen\x
  \pgfextractx{\x}{#1}
  \newdimen\y
  \pgfextracty{\y}{#1}
  \pgfpoint{-\y}{\x}
}

\def\hgperpr#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Compute a length-radius vector perpendicular (counter-clockwise)
  % to the line from start point to end point.
  \pgfpointscale{#3}{
    \hgrotate{
      \pgfpointnormalised{
        \pgfpointdiff{#1}{#2}}}}
}

\def\hgaddeperpr#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Add to end point a length-radius vector perpendicular
  % (counter-clockwise) to the line from start point to end point.
  \pgfpointadd{#2}{\hgperpr{#1}{#2}{#3}}
}

\def\hgaddsperpr#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Add to start point a length-radius vector perpendicular
  % (counter-clockwise) to the line from start point to end point.
  \pgfpointadd{\hgperpr{#1}{#2}{#3}}{#1}
}

\def\hgcorner#1#2#3#4{
  % #1 = previous point
  % #2 = current point
  % #3 = next point
  % #4 = radius
  % Draw a line to and a round corner on the outside of the angle #1#2#3.
  \pgflineto{\hgaddeperpr{#1}{#2}{#4}}
  \pgfmathanglebetweenpoints{#1}{#2}\let\anga\pgfmathresult
  % \pgfmathanglebetweenpoints{#2}{#3}\let\angb\pgfmathresult
  % \pgfpatharc{90 + \anga}{90 + \angb}{#4}
  \pgfpatharcto{#4}{#4}{90 + \anga}{0}{0}{\hgaddsperpr{#2}{#3}{#4}}
}

\def\hgedgeiiipriv#1#2#3#4{
  % #1#2#3 = pgf points
  % #4 = radius
  % Computes a path comprising the line of the points outside of the
  % convex hull H of the points #1#2#3 that have distance radius to H.
  % Points #1#2#3 need to be in clockwise order.
  \pgfpathmoveto{\hgaddeperpr{#3}{#1}{#4}}
  \hgcorner{#3}{#1}{#2}{#4}
  \hgcorner{#1}{#2}{#3}{#4}
  \hgcorner{#2}{#3}{#1}{#4}
  \pgfpathclose
}

\def\hgedgeiii#1#2#3#4{
  % #1#2#2 = pgf nodes
  % #4 = radius
  % Computes a path comprising the line of the points outside of the
  % convex hull H of the points #1#2#3 that have distance radius to H.
  % Points #1#2#3 need to be in clockwise order.
  \hgedgeiiipriv{
    \pgfpointanchor{#1}{center}}{
    \pgfpointanchor{#2}{center}}{
    \pgfpointanchor{#3}{center}}{
    #4}
}

\def\hgedgeiipriv#1#2#3{
  % #1#2 = pgf points
  % #3 = radius
  \pgfpathmoveto{\hgaddeperpr{#2}{#1}{#3}}
  \pgfpatharcto{#3}{#3}{90}{0}{0}{\hgaddsperpr{#1}{#2}{#3}}
  \pgflineto{\hgaddeperpr{#1}{#2}{#3}}
  \pgfpatharcto{#3}{#3}{270}{0}{0}{\hgaddsperpr{#2}{#1}{#3}}
  \pgfpathclose
}

\def\hgedgeii#1#2#3{
  \hgedgeiipriv{
    \pgfpointanchor{#1}{center}}{
    \pgfpointanchor{#2}{center}}{
    #3}
}


